MaAST: Map Attention with Semantic Transformersfor Efficient Visual Navigation

Visual navigation for autonomous agents is a core task in the fields of computer vision and robotics. Learning-based methods, such as deep reinforcement learning, have the potential to outperform the classical solutions developed for this task; however, they come at a significantly increased computational load. Through this work, we design a novel approach that focuses on performing better or comparable to the existing learning-based solutions but under a clear time/computational budget. To this end, we propose a method to encode vital scene semantics such as traversable paths, unexplored areas, and observed scene objects -- alongside raw visual streams such as RGB, depth, and semantic segmentation masks -- into a semantically informed, top-down egocentric map representation. Further, to enable the effective use of this information, we introduce a novel 2-D map attention mechanism, based on the successful multi-layer Transformer networks. We conduct experiments on 3-D reconstructed indoor PointGoal visual navigation and demonstrate the effectiveness of our approach. We show that by using our novel attention schema and auxiliary rewards to better utilize scene semantics, we outperform multiple baselines trained with only raw inputs or implicit semantic information while operating with an 80% decrease in the agent's experience.

==> defines_back.tex <==
\usepackage[font=small,labelfont=bf]{caption}
\usepackage[width=122mm,left=12mm,paperwidth=146mm,height=193mm,top=12mm,paperheight=217mm]{geometry}
\usepackage{subcaption}
\usepackage{wrapfig}
%\usepackage{times}
\usepackage{microtype}
\frenchspacing
\usepackage{xspace}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{amsmath, bm}
\usepackage{amssymb}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{mathtools}
\usepackage{array}
\usepackage{multirow}
\usepackage[inline]{enumitem}
\usepackage{multirow}
\usepackage{tabularx}
\usepackage{color}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage[hyphens]{url}   % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}
\usepackage{rotating}
\usepackage{lipsum}
\usepackage{wrapfig}
%\usepackage{blindtext}
%\usepackage{tikz}
\usepackage[numbers,sort]{natbib}
\usepackage{flushend}
% \usepackage{unicode-math}
\usepackage{cool}
\usepackage{siunitx}
\usepackage{bbm}

\setlength{\dbltextfloatsep}{7pt plus 1.0pt minus 2.0pt}
\setlength{\textfloatsep}{7pt plus 1.0pt minus 2.0pt}

% Include other packages here, before hyperref.

% If you comment hyperref and then uncomment it, you should delete
% egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% run, let it finish, and you should be clear).
\usepackage[pagebackref=true,breaklinks=true,colorlinks,bookmarks=false]{hyperref}
\usepackage[capitalise,nameinlink]{cleveref}
\newcommand{\crefrangeconjunction}{--}
\makeatletter
\crefname{section}{\S\@gobble}{\S\S\@gobble}
\Crefname{section}{\S\@gobble}{\S\S\@gobble}
\makeatother
% \cvprfinalcopy % *** Uncomment this line for the final submission

% \def\cvprPaperID{8388} % *** Enter the CVPR Paper ID here
% \def\httilde{\mbox{\tt\raisebox{-.5ex}{\symbol{126}}}}
% Pages are numbered in submission mode, and unnumbered in camera-ready
% \ifcvprfinal\pagestyle{empty}\fi

\DeclareMathOperator{\softmax}{softmax}

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\makeatother

\def\etal{\emph{et al}\onedot}
\def\etc{\emph{etc}\onedot}
\def\ie{\emph{i.e}\onedot}
\def\eg{\emph{e.g}\onedot}
\def\cf{\emph{cf}\onedot}
\def\vs{\emph{vs}\onedot}
\def\viz{\emph{viz}\onedot}
\def\pd{\partial}
\def\grad{\nabla}
\def\R{\mathbb{R}}
\def\d{\boldsymbol{\delta}}
\def\y{\textbf{y}}
\def\l{\boldsymbol{\ell}}
\def\wrt{with regard to\xspace}
\def\a{\boldsymbol{\alpha}}
\def\vertspace{0.6em}
\newcommand{\mat}[1]{\bm{#1}}

%Defining matrices and vector notations as per goodfellows book
\def\mF{\mat{F}}
\def\mM{\mat{M}}
\def\mW{\mat{W}}
\def\mI{\mat{I}}
\def\conv{\circledast}


\definecolor{redcol}{rgb}{1, 0, 0}
\definecolor{bluecol}{rgb}{0, 0, 1}
\newcommand{\red}[1]{\textcolor{redcol}{#1}} 
\newcommand{\blue}[1]{\textcolor{bluecol}{#1}} 
\renewcommand{\paragraph}[1]{\smallskip\noindent{\bf{#1}}}
\newcommand{\mast}[0]{MaAST\xspace}
%%%%%%%%%%%

\newcommand{\habitatsim}{\texttt{Habitat-Sim}\xspace}
\newcommand{\habitatapi}{\texttt{Habitat-API}\xspace}
\newcommand{\spl}{\texttt{SPL}\xspace}
\newcommand{\blind}{\texttt{Blind}\xspace}
\newcommand{\rgb}{\texttt{RGB}\xspace}
\newcommand{\depth}{\texttt{Depth}\xspace}
\newcommand{\rgbd}{\texttt{RGB-D}\xspace}
\newcommand{\rgbdocc}{\texttt{RGBD+OCC}\xspace}
\newcommand{\rgbdexp}{\texttt{RGBD+EXP}\xspace}
\newcommand{\rgbdsem}{\texttt{RGBD+SEM}\xspace}
\newcommand{\depthsem}{\texttt{DEPTH+SEM}\xspace}
\newcommand{\occatt}{\texttt{RGBD+OCC+ATT}\xspace}
\newcommand{\rgbdatt}{\mast}
\newcommand{\rgbdroom}{\texttt{RGBD+ROOM}\xspace}
\newcommand{\todoblue}[1]{\textcolor{blue}{#1}}
\newcommand{\train}{\texttt{train}\xspace}
\newcommand{\val}{\texttt{val}\xspace}
\newcommand{\minival}{\texttt{mini-val}\xspace}
\newcommand{\test}{\texttt{test}\xspace}
\newcommand{\leftaction}{\texttt{Turn Left}\xspace}
\newcommand{\rightaction}{\texttt{Turn Right}\xspace}
\newcommand{\forwardaction}{\texttt{Move Forward}\xspace}
\newcommand{\stopaction}{\texttt{STOP}\xspace}
\DeclareSIUnit{\million}{\text{milion}}

==> tables/ablation.tex <==
\begin{table*}[t]
  \centering
  \footnotesize
   \caption{Ablation study of the proposed \mast method on the Matterport3D validation set. All models are evaluated after training for 14 million steps of experience using RL (PPO). $\mathbf{\dagger}$: uses our egocentric map Transformer.}
%   \begin{tabular}{@{} p{0.8in} p{0.6in} cccc@{}}
\scalebox{0.74}{
\begin{tabular}{lcccccccccc}
      \toprule
      & & \multicolumn{3}{c}{Sensors} & & \multicolumn{2}{c}{Rewards} & & \\
      \cmidrule{3-6} \cmidrule{7-8}
      \multicolumn{2}{c}{Method} & RGB & Depth & Semantic & Map & Goal & Exploration & \spl(\%) & Succ(\%) \\
      \midrule
     \multirow{1}{*}{\mast w/o \texttt{(EXP,SEM,ATT)}}
      & \rgbd   & $\checkmark$ & $\checkmark$ & & & $\checkmark$ &  &  $34$ & $51$ \\
      \multirow{1}{*}{\mast w/o \texttt{(SEM,ATT)}}
      & \rgbdexp & $\checkmark$ & $\checkmark$ & & & $\checkmark$ & $\checkmark$ &  $38$ & $53$ \\
      \multirow{1}{*}{\mast w/o \texttt{ATT}}
      & \rgbdsem & $\checkmark$ & $\checkmark$ & $\checkmark$ & Semantic & $\checkmark$ & $\checkmark$ & $41$ & $49$ \\
      \multirow{1}{*}{\mast w/o \texttt{SEM}, + \texttt{OCC}}
      & \occatt & $\checkmark$ & $\checkmark$ & & Occupancy$\dagger$ & $\checkmark$ & $\checkmark$ & $44$ & $52$ \\
      \multirow{1}{*}{\mast}
      & \texttt{RGBD+SEM+ATT}  & $\checkmark$ & $\checkmark$ & $\checkmark$ & Semantic$\dagger$  & $\checkmark$ & $\checkmark$ & \textbf{47} & \textbf{54} \\
      \bottomrule
  \end{tabular}}
 %}

  \label{tab:ablation}
%  \vspace{\captionReduceBot}
\end{table*}



==> tables/mp3d.tex <==


\begin{table*}[t]
\vspace{0.2cm}
  \centering
   \caption{Results of our proposed method, compared against several alternatives, evaluated for visual navigation on the Matterport3D validation set. We report both success weighted by path length (\spl) and episode success rate. $\mathbf{\dagger}$: uses our egocentric map Transformer.}
   \vspace{-0.2cm}
  \footnotesize
%   \begin{tabular}{@{} p{0.8in} p{0.6in} cccc@{}}
\scalebox{0.73}{
\begin{tabular}{llccccccccc}

      \toprule
      & & & \multicolumn{3}{c}{Sensors} & & \multicolumn{2}{c}{Rewards} & & \\
      \cmidrule{4-7} \cmidrule{8-9}
      \multicolumn{2}{c}{Method} & Experience (Steps) & RGB & Depth & Semantic & Map & Goal & Exploration & \spl(\%) & Succ(\%) \\
      \midrule
      \multirow{4}{*}{\blind~\cite{habitat19iccv}}
      & Random & - & & & & & & & $01$ & $01$  \\
      & Forward only & - & & & & & & &$00$ & $00$  \\
      & Goal follower & - & & & & & & & $12$ & $12$   \\
      & RL (PPO) & \SI{75}{\million} & & & & & $\checkmark$ & & $25$ & $35$  \\
      \midrule
    %   \multirow{1}{*}{\rgb}
    %   & RL (PPO) & $\checkmark$ & & & & & & $-$ & $-$ \\
    %   \multirow{1}{*}{\depth}
    %   & RL (PPO) & & $\checkmark$ & & & & & $-$ & $-$ \\
      \multirow{1}{*}{\rgbd~\cite{habitat19iccv}}
      & RL (PPO) & \SI{14}{\million} & $\checkmark$ & $\checkmark$ & &  & $\checkmark$ & & $34$ & $51$  \\
      \multirow{1}{*} {\rgbd~\cite{habitat19iccv}}& SLAM & - & $\checkmark$ & $\checkmark$ & & & & & $42$ & - \\
    %   \multirow{1}{*}{\texttt{Situational Fusion}}
    %   & RL (PPO) & $\checkmark$ & $\dagger$ & $\dagger$ &  & $\checkmark$ & &  $-$ & $-$ \\
     % \midrule
    %   \multirow{1}{*}{\rgbdexp}
    %   & RL (PPO) & \SI{14}{\million} & $\checkmark$ & $\checkmark$ & & & $\checkmark$ & $\checkmark$ &  $0.38$ & $0.53$ \\
      \multirow{1}{*}{\rgbdocc~\cite{exp4nav}}
      & RL (PPO) & \SI{14}{\million} & $\checkmark$ & $\checkmark$ & & Occupancy & $\checkmark$ & $\checkmark$ &  $43$ & $52$ \\
    %   \multirow{1}{*}{\rgbdroom}
    %   & RL (PPO) & $\checkmark$ & $\checkmark$ & $\checkmark$ &  & $\checkmark$ & Room &  $0.36$ & $0.53$ \\
    %   \multirow{1}{*}{\rgbdsem}
    %   & RL (PPO) & \SI{14}{\million} & $\checkmark$ & $\checkmark$ & $\checkmark$ & Semantic & $\checkmark$ & $\checkmark$ & $0.41$ & $0.49$ \\
    %   \multirow{1}{*}{\occatt}
    %   & RL (PPO) & \SI{14}{\million} & $\checkmark$ & $\checkmark$ & & Occupancy$\dagger$ & $\checkmark$ & $\checkmark$ & $0.44$ & $0.52$ \\
      \multirow{1}{*}{\mast}
      & RL (PPO) & \SI{14}{\million} & $\checkmark$ & $\checkmark$ & $\checkmark$ & Semantic$\dagger$  & $\checkmark$ & $\checkmark$ & \textbf{47} & \textbf{54} \\
      \bottomrule
  \end{tabular}}

  \label{tab:baselines}
%  \vspace{\captionReduceBot}
\end{table*}


% \begin{table}
%   \centering
%   \footnotesize
%   \begin{tabular}{@{} p{0.8in} p{0.6in} cccccc@{}}
%       \toprule
%       & & \multicolumn{2}{c}{Gibson} & \multicolumn{2}{c}{MP3D} \\
%       \cmidrule(l){3-4} \cmidrule(l){5-6}  \cmidrule(l){7-8}
%       Sensors & Baseline & SPL & Succ & SPL & Succ \\
%       \midrule
%       %\cmidrule{1-8}
%       \multirow{4}{*}{\blind}
%       & Random & $0.02$ & $0.03$ & $0.01$ & $0.01$  \\
%       & Forward only & $0.00$ & $0.00$ & $0.00$ & $0.00$  \\
%       & Goal follower & $0.23$ & $0.23$ & $0.12$ & $0.12$   \\
%       & RL (PPO) & $0.42$ & $0.62$ & $0.25$ & $0.35$  \\
%       \midrule
%       %\cmidrule{2-8}
%       \multirow{1}{*}{\rgb}
%       & RL (PPO) & $0.46$ & $0.64$ & $0.30$ & $0.42$ \\
%       \midrule
%       %\cmidrule{2-8}
%       \multirow{1}{*}{\depth}
%       & RL (PPO) & $\textbf{0.79}$ & $\textbf{0.89}$ & $\textbf{0.54}$ & $\textbf{0.69}$ \\
%       \midrule
%       %\cmidrule{2-8}
%       \multirow{2}{*}{\rgbd}
%       & RL (PPO) & $0.70$ & $0.80$ & $0.42$ & $0.53$  \\
%       & SLAM~\cite{Mishkin2019BenchmarkingCA} & $0.51$ & $0.62$ & $0.39$ & $0.47$ \\
%       \multirow{1}{*}{\rgbdocc}
%       & RL (PPO)  & $-$ & $-$ & $-$ & $-$ \\
%       \multirow{1}{*}{\rgbdsem}
%       & RL (PPO)  & $-$ & $-$ & $-$ & $-$ \\
%       \multirow{1}{*}{\rgbdatt}
%       & RL (PPO)  & $-$ & $-$ & $-$ & $-$ \\
      
%       \bottomrule
%   \end{tabular}\\[3pt]
% %   
%   \label{tab:baselines}
% %  \vspace{\captionReduceBot}
% \end{table}

% \begin{table}[t]
%   \centering
%   \scriptsize
% %   \begin{tabular}{@{} p{0.8in} p{0.6in} cccc@{}}
% \caption{Results of our proposed method, compared against several alternatives, evaluated for visual navigation on the Matterport3D test split. We report both success weighted by path length (\spl) and episode success rate after training all models for 10 million steps following~\cite{anm20iclr}}
% \begin{tabular}{lcccccccc}
%       \toprule
%       & \multicolumn{4}{c}{Sensors} & \multicolumn{2}{c}{Rewards} & & \\
%       \cmidrule{2-5} \cmidrule{6-7}
%       Method & RGB & Depth & Semantic & Map & Goal & Exploration & \spl & Succ \\
%       \midrule
%       Random & & & & & & & $0.010$ & $0.010$  \\
%       %& Forward only & - & & & & & & &$0.00$ & $0.00$  \\
%       %& Goal follower & - & & & & & & & $0.12$ & $0.12$   \\
%       Blind + RL (PPO) & & & & & $\checkmark$ & & $0.087$ & $0.136$  \\
%       \midrule
%     %   \multirow{1}{*}{\rgb}
%     %   & RL (PPO) & $\checkmark$ & & & & & & $-$ & $-$ \\
%     %   \multirow{1}{*}{\depth}
%     %   & RL (PPO) & & $\checkmark$ & & & & & $-$ & $-$ \\
     
%       RL + Res18~\cite{anm20iclr} & $\checkmark$ & & &  & $\checkmark$ & & $0.125$ & $0.160$  \\
%       %IL + Res18~\cite{anm20iclr} & $\checkmark$ & & &  & $\checkmark$ & & $0.318$ & $0.365$  \\
%       %\midrule
%       RL + 3LConv~\cite{habitat19iccv} & $\checkmark$ & & &  & $\checkmark$ & $\checkmark$& $0.080$ & $0.102$  \\
%       RL + Res18 + AuxDepth~\cite{anm20iclr} & $\checkmark$ & & &  & $\checkmark$ & & $0.143$ & $0.189$  \\
%       RL + Res18 + ProjDepth~\cite{anm20iclr} & $\checkmark$ & & & Occupancy & $\checkmark$ & & $0.111$ & $0.134$  \\
%       CMP~\cite{anm20iclr} & $\checkmark$ & & & Confidence & $\checkmark$ & & $0.270$ & $0.320$  \\
%       %& SLAM & - & $\checkmark$ & $\checkmark$ & & & & & $0.42$ & - \\
%     %   \multirow{1}{*}{\texttt{Situational Fusion}}
%     %   & RL (PPO) & $\checkmark$ & $\dagger$ & $\dagger$ &  & $\checkmark$ & &  $-$ & $-$ \\
%       \midrule
%       RL + 3LConv + ProjDepth & $\checkmark$ & $\checkmark$ & & Occupancy & $\checkmark$ & $\checkmark$ & $0.295$ & $0.357$ \\
%       RL + 3LConv + \mast (Ours) & $\checkmark$ & $\checkmark$ & $\checkmark$& Semantic & $\checkmark$ & $\checkmark$ & \textbf{0.334} & \textbf{0.404} \\
%       \bottomrule
%   \end{tabular}
 
%   \label{tab:baselines}
% %  \vspace{\captionReduceBot}
% \end{table}



==> tables/mp3d_with_ANM.tex <==

% \begin{table}
%   \centering
%   \footnotesize
%   \begin{tabular}{@{} p{0.8in} p{0.6in} cccccc@{}}
%       \toprule
%       & & \multicolumn{2}{c}{Gibson} & \multicolumn{2}{c}{MP3D} \\
%       \cmidrule(l){3-4} \cmidrule(l){5-6}  \cmidrule(l){7-8}
%       Sensors & Baseline & SPL & Succ & SPL & Succ \\
%       \midrule
%       %\cmidrule{1-8}
%       \multirow{4}{*}{\blind}
%       & Random & $0.02$ & $0.03$ & $0.01$ & $0.01$  \\
%       & Forward only & $0.00$ & $0.00$ & $0.00$ & $0.00$  \\
%       & Goal follower & $0.23$ & $0.23$ & $0.12$ & $0.12$   \\
%       & RL (PPO) & $0.42$ & $0.62$ & $0.25$ & $0.35$  \\
%       \midrule
%       %\cmidrule{2-8}
%       \multirow{1}{*}{\rgb}
%       & RL (PPO) & $0.46$ & $0.64$ & $0.30$ & $0.42$ \\
%       \midrule
%       %\cmidrule{2-8}
%       \multirow{1}{*}{\depth}
%       & RL (PPO) & $\textbf{0.79}$ & $\textbf{0.89}$ & $\textbf{0.54}$ & $\textbf{0.69}$ \\
%       \midrule
%       %\cmidrule{2-8}
%       \multirow{2}{*}{\rgbd}
%       & RL (PPO) & $0.70$ & $0.80$ & $0.42$ & $0.53$  \\
%       & SLAM~\cite{Mishkin2019BenchmarkingCA} & $0.51$ & $0.62$ & $0.39$ & $0.47$ \\
%       \multirow{1}{*}{\rgbdocc}
%       & RL (PPO)  & $-$ & $-$ & $-$ & $-$ \\
%       \multirow{1}{*}{\rgbdsem}
%       & RL (PPO)  & $-$ & $-$ & $-$ & $-$ \\
%       \multirow{1}{*}{\rgbdatt}
%       & RL (PPO)  & $-$ & $-$ & $-$ & $-$ \\
      
%       \bottomrule
%   \end{tabular}\\[3pt]
% %   
%   \label{tab:baselines}
% %  \vspace{\captionReduceBot}
% \end{table}

\begin{table}[t]
  \centering
  \scriptsize
%   \begin{tabular}{@{} p{0.8in} p{0.6in} cccc@{}}
\caption{Results of our proposed method, compared against several alternatives, evaluated for visual navigation on the Matterport3D test split. We report both success weighted by path length (\spl) and episode success rate after training all models for 10 million steps following~\cite{anm20iclr}}
\begin{tabular}{lcccccccc}
      \toprule
      & \multicolumn{4}{c}{Sensors} & \multicolumn{2}{c}{Rewards} & & \\
      \cmidrule{2-5} \cmidrule{6-7}
      Method & RGB & Depth & Semantic & Map & Goal & Exploration & \spl & Succ \\
      \midrule
      Random & & & & & & & $0.010$ & $0.010$  \\
      %& Forward only & - & & & & & & &$0.00$ & $0.00$  \\
      %& Goal follower & - & & & & & & & $0.12$ & $0.12$   \\
      Blind + RL (PPO) & & & & & $\checkmark$ & & $0.087$ & $0.136$  \\
      \midrule
    %   \multirow{1}{*}{\rgb}
    %   & RL (PPO) & $\checkmark$ & & & & & & $-$ & $-$ \\
    %   \multirow{1}{*}{\depth}
    %   & RL (PPO) & & $\checkmark$ & & & & & $-$ & $-$ \\
     
      RL + Res18~\cite{anm20iclr} & $\checkmark$ & & &  & $\checkmark$ & & $0.125$ & $0.160$  \\
      %IL + Res18~\cite{anm20iclr} & $\checkmark$ & & &  & $\checkmark$ & & $0.318$ & $0.365$  \\
      %\midrule
       RL + 3LConv~\cite{habitat19iccv} & $\checkmark$ & & &  & $\checkmark$ & $\checkmark$& $0.080$ & $0.102$  \\
      RL + Res18 + AuxDepth~\cite{anm20iclr} & $\checkmark$ & & &  & $\checkmark$ & & $0.143$ & $0.189$  \\
      RL + Res18 + ProjDepth~\cite{anm20iclr} & $\checkmark$ & & & Occupancy & $\checkmark$ & & $0.111$ & $0.134$  \\
      CMP~\cite{anm20iclr} & $\checkmark$ & & & Confidence & $\checkmark$ & & $0.270$ & $0.320$  \\
      %& SLAM & - & $\checkmark$ & $\checkmark$ & & & & & $0.42$ & - \\
    %   \multirow{1}{*}{\texttt{Situational Fusion}}
    %   & RL (PPO) & $\checkmark$ & $\dagger$ & $\dagger$ &  & $\checkmark$ & &  $-$ & $-$ \\
      \midrule
      RL + 3LConv + ProjDepth & $\checkmark$ & $\checkmark$ & & Occupancy & $\checkmark$ & $\checkmark$ & $0.295$ & $0.357$ \\
       RL + 3LConv + \mast (Ours) & $\checkmark$ & $\checkmark$ & $\checkmark$& Semantic & $\checkmark$ & $\checkmark$ & \textbf{0.334} & \textbf{0.404} \\
      \bottomrule
  \end{tabular}
 
  \label{tab:baselines}
%  \vspace{\captionReduceBot}
\end{table}


